Large Language Model is Secretly a Protein Sequence Optimizer

We consider the protein sequence engineering problem, which aims to find protein sequences with high fitness levels, starting from a given wild-type sequence. Directed evolution has been a dominating paradigm in this field which has an iterative process to generate variants and select via experimental feedback. We demonstrate large language models (LLMs), despite being trained on massive texts, are secretly protein sequence optimizers. With a directed evolutionary method, LLM can perform protein engineering through Pareto and experiment-budget constrained optimization, demonstrating success on both synthetic and experimental fitness landscapes.

==> figures/box_plot.tex <==
\begin{figure}[ht]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.3\textwidth]{figures/GB1_box_96_seed1.png} & 
\includegraphics[width=0.3\textwidth]{figures/Syn-3bfo_box_96_seed1.png} &
\includegraphics[width=0.3\textwidth]{figures/AAV_box_96_seed1.png} \\
(a) GB1  & (b) Syn-3bfo & (c) AAV  \\[6pt]
\end{tabular}
\caption{Fitness score for landscape GB1, Syn-3bfo, AAV among all iteration for EA and our framework.}
\label{fig:boxplots_datasets}
\end{figure}

==> tables/constrain.tex <==

\begin{table}[ht]
\centering
\begin{tabular}{cccccc}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Method} & \multirow{3}{*}{H} & \multicolumn{3}{c}{Metric} \\ \cmidrule{4-6}
                         &                        &                                  & Top 1 & Top 10 & Top 50 \\ \midrule
                        \multirow{6}{*}{Syn-3bfo}     & \multirow{3}{*}{EA} &   
                        3    & 1.06(0.12)    & 0.12(0.27)    & -1.01(0.35)   \\
                         & & 5& 1.28(0.59)    & 0.34(0.45)    & -0.86(0.12) \\
                         & & 10 &  1.28(0.59)    & 0.34(0.45)    & -0.86(0.12)\\
                         \cmidrule{2-6}
                         & \multirow{3}{*}{Ours} & 3    & 0.34(0.06)    & -0.47(0.27)    & -1.41(0.45)   \\
                         & & 5& 2.09(0.25)    & 0.66(0.59)    & -0.65(0.65) \\
                         & & 10 & 2.03(0.18)    & 1.35(0.12)    & -0.14(0.31)\\
                        \bottomrule
\end{tabular}
\caption{Experimental results for constrained optimization. The population size is 48 while the iteration is 8. H refers to the hamming distance constrain between proposed sequence and the wild type sequence.} 
\label{tab:constrain_result}
\end{table}
